Keystroke Verification Challenge (KVC): Biometric and Fairness Benchmark Evaluation

Analyzing keystroke dynamics (KD) for biometric verification has several advantages: it is among the most discriminative behavioral traits; keyboards are among the most common human-computer interfaces, being the primary means for users to enter textual data; its acquisition does not require additional hardware, and its processing is relatively lightweight; and it allows for transparently recognizing subjects. However, the heterogeneity of experimental protocols and metrics, and the limited size of the databases adopted in the literature impede direct comparisons between different systems, thus representing an obstacle in the advancement of keystroke biometrics. To alleviate this aspect, we present a new experimental framework to benchmark KD-based biometric verification performance and fairness based on tweet-long sequences of variable transcript text from over 185,000 subjects, acquired through desktop and mobile keyboards, extracted from the Aalto Keystroke Databases. The framework runs on CodaLab in the form of the Keystroke Verification Challenge (KVC). Moreover, we also introduce a novel fairness metric, the Skewed Impostor Ratio (SIR), to capture inter- and intra-demographic group bias patterns in the verification scores. We demonstrate the usefulness of the proposed framework by employing two state-of-the-art keystroke verification systems, TypeNet and TypeFormer, to compare different sets of input features, achieving a less privacy-invasive system, by discarding the analysis of text content (ASCII codes of the keys pressed) in favor of extended features in the time domain. Our experiments show that this approach allows to maintain satisfactory performance.

==> 8_Experimental_Results_old.tex <==

\subsection{Biometric Verification}
\label{subsec:biometric_verification}
The results of the experiments are reported in Table \ref{tab:all_metrics}. The table is divided into two parts, each one corresponding to one scenario: desktop and mobile. Each half can be further divided into the two cases considered: results obtained in the global genuine and impostor distributions (see Sec. \ref{sec:evaluation_description}), and results considering the mean values obtained for per-subject genuine and impostor distributions. Each row shows a different system, TypeNet or TypeFormer, trained on a different set of input features, according to the 4 experiments described in Sec. \ref{subsec:evaluation}, while the different metrics are reported along the columns.





% \begin{table}
% \caption{The confusion matrix for each of the cases presented.}
% \centering
% \begin{tabular}{|c|c||c|c|}
% \multicolumn{4}{c}{\textbf{Baseline RNN}} \\
% \multicolumn{2}{c}{Desktop} & \multicolumn{2}{c}{Mobile} \\
% \hline
%  \textbf{TN}: 49.98\% & \textbf{FP}: 16.69\% & \textbf{TN}: 44.44\% & \textbf{FP}: 22.23\% \\
% \hline
%  \textbf{FN}: 8.34\% & \textbf{TP}: 24.99\% & \textbf{FN}: 11.11\% & \textbf{TP}: 22.22\% \\
% \hline
% \end{tabular}

% % \vspace{.3cm}

% \begin{tabular}{|c|c||c|c|}
% \multicolumn{4}{c}{\textbf{TypeNet \cite{typenet}}} \\
% \multicolumn{2}{c}{Desktop} & \multicolumn{2}{c}{Mobile} \\
% \hline
%  \textbf{TN}: 62.16\% & \textbf{FP}: 4.51\% & \textbf{TN}: 57.36\% & \textbf{FP}: 9.30\% \\
% \hline
%  \textbf{FN}: 2.25\% & \textbf{TP}: 31.08\% & \textbf{FN}: 4.65\% & \textbf{TP}: 28.68\% \\
% \hline
% \end{tabular}

% % \vspace{.3cm}

% \begin{tabular}{|c|c||c|c|}
% \multicolumn{4}{c}{\textbf{TypeFormer \cite{typeformer}}} \\
% \multicolumn{2}{c}{Desktop} & \multicolumn{2}{c}{Mobile} \\
% \hline
%  \textbf{TN}: 58.39\% & \textbf{FP}: 8.27\% & \textbf{TN}: 60.44\% & \textbf{FP}: 6.23\% \\
% \hline
%  \textbf{FN}: 4.14\% & \textbf{TP}: 29.20\% & \textbf{FN}: 3.11\% & \textbf{TP}: 30.22\% \\
% \hline
% \end{tabular}
% \label{tab:confusion_matrix}
% \end{table}

% , used to generate the challenge ranking: it is computed by considering the entire distributions of genuine and impostor scores. This is the only score that will be made public during the challenge. The remaining metrics will be published in the summary paper.
% Per-subject average EER: it is computed by considering subject-specific distributions of genuine and impostor scores, in other words, a different threshold per subject. By doing so, one EER per subject is obtained, then the mean value of all subject-specific EERs is considered.



\begin{table*}[hbt!]
\centering
\scriptsize
\caption{\small  Complete comparison of the presented keystroke biometric verification systems.}
\begin{tabular}{P{0.11\textwidth}|P{0.1\textwidth}|P{0.1\textwidth}|P{0.1\textwidth}|P{0.1\textwidth}}
\multicolumn{5}{c}{\textbf{Desktop}} \\
\bottomrule
\multicolumn{5}{c}{Global Distributions} \\
\bottomrule
\textbf{Experiment} & 
\textbf{EER$\downarrow$ (\%)} & 
\makecell{\textbf{FNMR$\downarrow$ @1\%}\\ \textbf{FMR (\%)}} & 
\makecell{\textbf{FNMR$\downarrow$ @10\%}\\ \textbf{FMR (\%)}} &
\textbf{AUC$\uparrow$ (\%)} \\
\bottomrule
\textbf{TypeNet, \textit{5F}} & \textbf{6.76} & \textbf{39.57} & \textbf{3.45} & \textbf{98.08}  \\
TypeNet, \textit{4F}  & 8.97 & 52.17 & 7.56 & 96.92  \\
TypeNet, \textit{10F}  & 8.95 & 51.57 & 7.51 & 96.91 \\
TypeNet, \textit{11F}  & 6.88 & 40.0 & 3.64 & 98.02 \\
\textbf{Average}  & \textbf{7.89} & \textbf{45.83} & \textbf{5.54} & \textbf{97.48} \\
\hline
TypeFormer, \textit{5F} & 12.92 & 75.51 & 18.93 & 94.15  \\
TypeFormer, \textit{4F} & 14.05 & 76.28 & 22.22 & 93.37  \\
TypeFormer, \textit{10F} & 12.75 & 73.51 & 18.19 & 94.31 \\
TypeFormer, \textit{11F} & 12.92 & 75.51 & 18.93 & 94.15 \\
\textbf{Average} & \textbf{13.17} & \textbf{75.10} & \textbf{19.59} & \textbf{93.98} \\
\bottomrule

% &  \makecell{\textbf{Rank-3$\uparrow$}\\ \textbf{(\%)}} &  \makecell{\textbf{Rank-5$\uparrow$}\\ \textbf{(\%)}}  
\end{tabular}
\begin{tabular}{P{0.11\textwidth}|P{0.1\textwidth}|P{0.1\textwidth}|P{0.1\textwidth}}
\multicolumn{4}{c}{Mean Per-Subject Distributions} \\
\bottomrule
\textbf{Experiment} & \textbf{EER$\downarrow$ (\%)} & \makecell{\textbf{AUC$\uparrow$}\\  \textbf{(\%)}} & \makecell{\textbf{Rank-1$\uparrow$}\\\textbf{(\%)}} \\
\bottomrule
\textbf{TypeNet, \textit{5F}}  & \textbf{2.71} & \textbf{99.26} & \textbf{89.81} \\
TypeNet, \textit{4F}  & 4.13 & 98.67 & 83.46 \\
TypeNet, \textit{10F} & 4.16 & 98.66 & 83.58\\
TypeNet, \textit{11F} & 2.76 & 99.24 & 89.52\\
\textbf{Average} & \textbf{3.44} & \textbf{98.96} & \textbf{86.59} \\

\hline
TypeFormer, \textit{5F}  & 7.76 & 96.51 & 65.52 
% & 91.58 & 97.43
\\
TypeFormer, \textit{4F} & 8.62 & 95.99 & 62.7 
% & 89.83 & 96.62
\\
TypeFormer, \textit{10F} & 7.4 & 96.77 & 67.72 
% & 92.41 & 97.63
\\
TypeFormer, \textit{11F} & 7.78 & 96.48 & 65.07 
% & 91.63 & 97.39
\\
\textbf{Average} & \textbf{7.89} & \textbf{96.44} & \textbf{65.25} \\

\bottomrule

\end{tabular}

\begin{tabular}{P{0.11\textwidth}|P{0.1\textwidth}|P{0.1\textwidth}|P{0.1\textwidth}|P{0.1\textwidth}}
\multicolumn{5}{c}{\textbf{Mobile}} \\
\bottomrule
\multicolumn{5}{c}{Global Distributions} \\
\bottomrule
\textbf{Experiment} & 
\textbf{EER$\downarrow$ (\%)} & 
\makecell{\textbf{FNMR$\downarrow$ @1\%}\\ \textbf{FMR (\%)}} & 
\makecell{\textbf{FNMR$\downarrow$ @10\%}\\ \textbf{FMR (\%)}} &
\textbf{AUC$\uparrow$ (\%)} \\
\bottomrule
TypeNet, \textit{5F}  & 13.95 & 70.05 & 22.22 & 93.8 \\
TypeNet, \textit{4F} & 16.36 & 76.64 & 28.52 & 91.41\\
TypeNet, \textit{10F} & 14.51 & 77.07 & 23.79 & 92.71\\
TypeNet, \textit{11F} & 14.8 & 68.16 & 23.48 & 93.71 \\
\textbf{Average}  & \textbf{14.91} & \textbf{72.98} & \textbf{24.50} & \textbf{92.91} \\
\hline

TypeFormer, \textit{5F} & 10.17 & 70.57 & 10.46 & 95.86 \\
TypeFormer, \textit{4F}   & 13.7 & 78.5 & 21.48 & 93.4 \\
\textbf{TypeFormer, \textit{10F}}  & \textbf{9.45} & \textbf{67.67} & \textbf{8.53} & \textbf{96.22} \\
TypeFormer, \textit{11F}  & 11.95 & 74.96 & 16.16 & 94.81 \\
\textbf{Average} & \textbf{11.32} & \textbf{72.92} & \textbf{14.16} & \textbf{95.07}  \\
\bottomrule

% &  \makecell{\textbf{Rank-3$\uparrow$}\\ \textbf{(\%)}} &  \makecell{\textbf{Rank-5$\uparrow$}\\ \textbf{(\%)}}  
\end{tabular}
\begin{tabular}{P{0.11\textwidth}|P{0.1\textwidth}|P{0.1\textwidth}|P{0.1\textwidth}}
\multicolumn{4}{c}{Mean Per-Subject Distributions} \\
\bottomrule
\textbf{Experiment} & \textbf{EER$\downarrow$ (\%)} & \makecell{\textbf{AUC$\uparrow$}\\  \textbf{(\%)}} & \makecell{\textbf{Rank-1$\uparrow$} \\ \textbf{(\%)}} 
% &  \makecell{\textbf{Rank-3$\uparrow$}\\ \textbf{(\%)}} &  \makecell{\textbf{Rank-5$\uparrow$}\\ \textbf{(\%)}}  
\\
\bottomrule
TypeNet, \textit{5F} & 7.99 & 96.43 & 68.5 \\
TypeNet, \textit{4F} & 9.64 & 95.46 & 65.13 \\
TypeNet, \textit{10F} & 8.3 & 96.19 & 66.15 \\
TypeNet, \textit{11F} & 7.99 & 96.54 & 68.49 \\
\textbf{Average}  & \textbf{8.48} & \textbf{96.16} & \textbf{67.07} \\
\hline
TypeFormer, \textit{5F}  & 5.92 & 97.45 & 71.3 
% & 94.82 & 98.6
\\
TypeFormer, \textit{4F} & 8.42 & 96.09 & 63.1 
% & 90.44 & 96.71
\\
\textbf{TypeFormer, \textit{10F}} & \textbf{5.25} & \textbf{97.89} & \textbf{75.92} 
% & \textbf{95.82} & \textbf{98.84} 
\\
TypeFormer, \textit{11F} & 7.41 & 96.66 & 66.04 
% & 92.0 & 97.68
\\
\textbf{Average} & \textbf{6.75} & \textbf{97.02} & \textbf{69.09} \\
\bottomrule
\end{tabular}
\vspace{0.2cm}
\label{tab:all_metrics}
\end{table*}

% Overall considerations: 
% - desktop better than mobile; OK
% - Case of different threshold per subject performs better OK
% - TypeNet better in the desktop case, TypeFormer better in the mobile case 
% (TAR at 1% FAR) and rank-1 
% 66, 33 max
% - TypeNet analysis of the features
% - TypeFormer analysis of the features

\begin{figure*}[hbt!]
\begin{center}
\begin{minipage}{\textwidth}

\captionsetup[sub]{labelformat=parens}
\captionsetup{type=figure}

\begin{subfigure}{.32\textwidth}
  \includegraphics[width=\linewidth]{images/distr_desktop.pdf}
     \caption{}
\end{subfigure}
\hfill
%\begin{subfigure}{.24\textwidth}
%  \includegraphics[width=\linewidth]{images/eer_curve_desktop.pdf}
%     \caption{}
% \end{subfigure}%
\hfill
\begin{subfigure}{.32\textwidth}
  \includegraphics[width=\linewidth]{images/det_desktop.pdf}
     \caption{}
\end{subfigure}%
 \hfill
\begin{subfigure}{.32\textwidth}
  \includegraphics[width=\linewidth]{images/roc_desktop.pdf}
 \caption{}
\end{subfigure}%
\hfill
\end{minipage}
\caption{The graphs show a comparison between \textbf{TypeNet} \textit{\textbf{5F}} \textbf{vs TypeNet} \textit{\textbf{10F}} in the desktop case. (a) shows the score histograms, (b) shows the DET curve, (c) shows the ROC curve.}
\label{fig:typenet_graphs}

\begin{minipage}{\textwidth}

\captionsetup[sub]{labelformat=parens}
\captionsetup{type=figure}

\begin{subfigure}{.32\textwidth}
  \includegraphics[width=\linewidth]{images/distr_mobile.pdf}
     \caption{}
\end{subfigure}
\hfill
%\begin{subfigure}{.24\textwidth}
%  \includegraphics[width=\linewidth]{images/eer_curve_mobile.pdf}
%     \caption{}
% \end{subfigure}%
% \hfill
\begin{subfigure}{.32\textwidth}
  \includegraphics[width=\linewidth]{images/det_mobile.pdf}
 \caption{}
\end{subfigure}%
\hfill
\begin{subfigure}{.32\textwidth}
  \includegraphics[width=\linewidth]{images/roc_mobile.pdf}
 \caption{}
\end{subfigure}%
\hfill
\end{minipage}
\caption{The graphs show a comparison between \textbf{TypeFormer} \textit{\textbf{5F}} \textbf{vs TypeFormer} \textit{\textbf{10F}} in the mobile case. (a) shows the score histograms, (b) shows the DET curve, (c) shows the ROC curve.}
\label{fig:typeformer_graphs}

% \centering
% \begin{minipage}{.24\textwidth}
%   \includegraphics[width=\linewidth]{images/distr_mobile.pdf}
% \end{minipage}
% \begin{minipage}{.24\textwidth}
%   \includegraphics[width=\linewidth]{images/eer_curve_mobile.pdf}
% \end{minipage}
% \begin{minipage}{.24\textwidth}
%   \includegraphics[width=\linewidth]{images/roc_mobile.pdf}
% \end{minipage}
% \label{fig:roc}
% \begin{minipage}{.24\textwidth}
%   \includegraphics[width=\linewidth]{images/det_mobile.pdf}
% \end{minipage}
% \caption{The Detection Error Tradeoff (DET) Curves in the desktop (left) and mobile (right) case.}
% \label{fig:det}
\end{center}
\end{figure*}


By observing the overall trends in the table, it is possible to notice that in the desktop case higher verification results can be achieved, possibly due to a more constrained acquisition scenario, as, in contrast to mobile devices, subjects are more likely to be sitting down and in a still position while typing on a desktop keyboard. In fact, as an example, considering both TypeNet and TypeFormer with all possible sets of features (8 experiments in total), the mean value of all EERs obtained from the global distributions in the desktop scenario is 10.53\%, whereas the corresponding value obtained in the mobile case is 13.11\%. The trend is consistent if we analyze the other metrics, such as the FNMR @1\% FMR (60.47\% vs 72.95\%) or AUC (95.73\% vs 93.99\%). %\footnote{The accuracy can be computed as the sum of TRR and TAR. Due to the design of the experimental protocol, with 10 genuine scores and 20 impostor scores per subject, the optimal values for TRR, FAR, FRR, TAR are respectively 66.7\%, 0\%, 0\%, 33.3\%.} 
Furthermore, the desktop case results to perform better also in the case of mean per-subject distributions. In this case, we obtain a mean EER of 5.67\% in the desktop case vs 7.61\% in the mobile case. Similarly, the mean AUC is 97.70\% vs 96.59\%, and the mean rank-1 is 75.92\% vs 68.08\%, respectively for desktop and mobile devices. 

Focusing on the four experiments involving different sets of input features, it is possible to draw some interesting conclusions. The best performing system for the desktop scenario is TypeNet, which is affected by the lack of the spatial information given by the ASCII code, and the extended set of features is not able to compensate it (6.76\% EER for TypeNet \textit{5F} vs 8.95\% EER for TypeNet \textit{10F} for global distributions). Nevertheless, despite the performance decrease, the system still shows competitive performance against the Transformer-based TypeFormer \textit{5F} or TypeFormer \textit{10F} (respectively 12.95\% EER and 12.75\% EER for global distributions). Moreover, these tendencies are consistent considering mean per-subject distributions.

The opposite outcome can be observed in the case of TypeFormer, which is the best performing system in the mobile case: the model achieved with the extended set of features (\textit{10F}) proves to be the best performing system in the mobile scenario (9.45\% EER vs second best, \textit{5F}, of 10.17\% EER for global distributions). Consequently, by introducing temporally-deepened input features, not only it has been possible to limit the performance decrease towards a more privacy-preserving verification system, but the verification performance is even significantly improved. In this case, it must be specified that the number of heads in the attention mechanism must be a multiple of the number of input features, consequently we considered (5 for \textit{5F} and \textit{10F}, 4 for \textit{4F}, and 1 for \textit{11F} due to memory constraints). In the case of TypeFormer, it is also interesting to point out that the second best performing model corresponds to the experiment \textit{5F}, with the initial set of features.

In addition, it is noticeable that subject-specific distributions lead to better verification performance in all cases. In fact, the system benefits from gaining more flexibility by setting a different threshold per subject. It is worth to highlight that this is really the case for security systems based on KD: in a real-life use case, once the system is deployed and the subject identity is verified in some other way, it is not hard to acquire multiple samples per subject. All these subject-specific data could be used as enrolment data, building a complete behavioral profile of the subject and leading to even better performance, without necessarily having to train or fine-tune the system. This would in fact be a further possible step, that leaves additional margin of improvement \cite{2018_INFFUS_MCSreview2_Fierrez}.

Another interesting observation is that it is very distinct how in the desktop case TypeNet performs better, while TypeFormer shows superiority in the mobile case. 
TypeNet is based on a two-layer LSTM RNN, while TypeFormer is based on a Transformer architecture, composed of several modules, and more parameters. 
As an example, in the desktop case the average TypeNet performance in terms of EER, FNMR @1\% FNMR, and AUC, over the four input feature experiments, is respectively 7.89\%, 45.83\%, 97.48\%, for global distributions and 3.44\% (EER), 98.96\% (AUC), 86.59\% (rank-1), for mean-per subject distributions. 
In each case, the corresponding values achieved by TypeFormer are 13.17\%, 75.10\%, 93.98\%, (global distributions), and 7.89\%, 96.44\%, 65.25\% (mean per-subject distributions), showing a significant gap. 
These trends are clearly opposite in the mobile case, where TypeFormer shows 11.32\%, 72.92\%, 95.07\% in the case of global distributions and 6.75\%, 97.02\%, 69.09\% for the mean per-subject distributions. 
In the corresponding experiments, TypeNet achieves 14.91\%, 72.98\%, 92.91\%, for global distributions and 8.48\%, 96.16\%, 67.07\% for the mean per-subject distributions. 
These trends show that LSTM RNNs seem to model well the desktop environment, while the higher variability of mobile devices is better modelled by a Transformer, which, however, does not reach the same level of performance in absolute terms.




In addition, in the case of the global distributions, also the FNMR @10\% FMR is reported. This represents a more relaxed approach, as the threshold selected is less stringent (90\% of the impostors are rejected against 99\% of FNMR @1\% FMR). According to both these metrics, TypeNet in the desktop case achieves significantly better results in comparison with all the other configurations, and its gap with TypeFormer is much greater than for the mobile case, where the two system performance is closer. These metrics are not computed for the case of mean per-subject distributions as there are not enough scores per subject for a sufficiently fine threshold resolution. They are substituted by the Rank-1 (not determinable for global distributions as subject-dependent), which also shows a more regular behavior of TypeNet in the desktop case in comparison with all other configurations.



Fig. \ref{fig:typenet_graphs} and Fig. \ref{fig:typeformer_graphs} show the curves described in Sec. \ref{subsec:curves}. In particular, it is possible to carry out a direct comparison of TypeNet in the desktop case and TypeFormer in the mobile case considering two of the four input feature sets presented above (\textit{5F} vs \textit{10F}). From left to right, the histograms of the genuine and impostor distributions are reported in Fig. \ref{fig:typenet_graphs} and \ref{fig:typeformer_graphs} (a). It is possible to see that in both rows the genuine distributions are more separated for the case of \textit{5F}, while for the mobile case (TypeFormer), the \textit{10F} setup is able to create a better separation of impostors, leading to a lower EER value. The threshold corresponding to the EER value is marked by the black line. From these macroscopic trends, the difference between the two impostor scenarios (``similar impostors'' and ``dissimilar impostors'', for comparison between subjects of the same and different demographic groups, respectively) is not very pronounced. In all graphs, the threshold values are reported in black. Then, Fig. \ref{fig:typenet_graphs} and \ref{fig:typeformer_graphs} (b) represent the DET curves (the threshold corresponding to 1\% and 10\% of FMR are respectively marked by the dashed red lines), while Fig. \ref{fig:typenet_graphs} and \ref{fig:typeformer_graphs} (c) report the ROC curves, showing similar trends from different perspectives.



\begin{table}[t]
\centering
\footnotesize 
\caption{\small Results in terms of Global EER for the final evaluation datasets (desktop and mobile), evaluated for the different demographic groups (gender and age). STD refers to the standard deviation, whereas SER refers to the Skewed Error Rate (Sec. \ref{sec:metrics}). Both metrics are computed from all the elements of each table.}
\label{table:bias}
\begin{tabular}{c|ccc}
\multicolumn{4}{c}{\textbf{TypeNet, \textit{5F}, Desktop, Global EER (\%)}} \\
\bottomrule
 & \textbf{Male} & \textbf{Female} & \textbf{Average} \\   
\hline
\textbf{10 - 13} & 6.04 & 6.38 & 6.21 \Tstrut\\
\textbf{14 - 17} & 6.62 & 7.01 & 6.81 \Tstrut\\
\textbf{18 - 26} & 6.27 & 6.78 & 6.53 \Tstrut\\
\textbf{27 - 35} & 6.74 & 7.33 & 7.04 \Tstrut\\
\textbf{36 - 44} & 7.01 & 7.47 & 7.24 \Tstrut\\
\textbf{45 - 79} & 6.74 & 7.69 & 7.22 \Tstrut\Bstrut\\
\textbf{Average} & 6.57 & 7.11 & - \\
\bottomrule
\multicolumn{4}{c}{\textbf{STD}: 0.27\%, \textbf{SER}: 1.34}\\
% \bottomrule
\end{tabular}
~\\~\\~\\
%\begin{tabular}{c|cc}
% \multicolumn{3}{c}{\textbf{TypeFormer, Desktop}} \\
% \bottomrule
%  & \textbf{Male} & \textbf{Female} \\   
% \hline
% \textbf{10 - 13} & 11.02 & 11.32 \Tstrut\\
% \textbf{14 - 17} & 12.71 & 12.88 \Tstrut\\
% \textbf{18 - 26} & 11.90 & 12.25 \Tstrut\\
% \textbf{27 - 35} & 12.32 & 13.32 \Tstrut\\
% \textbf{36 - 44} & 12.59 & 13.18 \Tstrut\\
% \textbf{45 - 79} & 12.23 & 13.44 \Tstrut\Bstrut\\
% \bottomrule
% \multicolumn{3}{c}{\textbf{STD}: 0.55\%, \textbf{SER}: 1.30}\\
% \bottomrule
%\end{tabular}\hspace{.5cm}
% \begin{tabular}{c|cc}
% \multicolumn{3}{c}{\textbf{TypeNet, \textit{5F}, Mobile}} \\
% \bottomrule
%  & \textbf{Male} & \textbf{Female} \\   
% \hline
% \textbf{10 - 13} & 14.85 & 15.63 \Tstrut\\
% \textbf{14 - 17} & 14.23 & 16.41 \Tstrut\\
% \textbf{18 - 26} & 12.70 & 14.60 \Tstrut\\
% \textbf{27 - 35} & 12.90 & 12.97 \Tstrut\\
% \textbf{36 - 44} & 12.11 & 12.34 \Tstrut\\
% \textbf{45 - 79} & 10.92 & 12.55 \Tstrut\Bstrut\\
% \bottomrule
% \multicolumn{3}{c}{\textbf{STD}: 1.36\%, \textbf{SER}: 1.93}\\
% \bottomrule
% \end{tabular}\hspace{.5cm}
\begin{tabular}{c|ccc}
\multicolumn{4}{c}{\textbf{TypeFormer, \textit{5F}, Mobile, Global EER (\%)}} \\
\bottomrule
 & \textbf{Male} & \textbf{Female} & \textbf{Average} \\   
\hline
\textbf{10 - 13} & 10.61 & 11.63 & 11.12 \Tstrut\\
\textbf{14 - 17} & 10.24 & 11.93 & 11.09 \Tstrut\\
\textbf{18 - 26} & 9.10 & 10.51 & 9.81 \Tstrut\\
\textbf{27 - 35} & 9.78 & 9.48 & 9.63 \Tstrut\\
\textbf{36 - 44} & 9.33 & 8.96 & 9.13 \Tstrut\\
\textbf{45 - 79} & 8.64 & 9.73 & 9.19 \Tstrut\Bstrut\\
\textbf{Average} & 9.62 & 10.37 & - \\
\bottomrule
\multicolumn{4}{c}{\textbf{STD}: 0.95\%, \textbf{SER}: 1.73}\\
% \bottomrule
\end{tabular}
% \vspace{0.2cm}
\label{tab:glob_eer_dem}
\end{table}

\begin{table*}[h!]
\scriptsize
\caption{Comparison of the presented keystroke biometric verification systems from the point of view of fairness metrics.}
\begin{tabular}{P{0.11\textwidth}|P{0.07\textwidth}|P{0.07\textwidth}|P{0.07\textwidth}|P{0.07\textwidth}|P{0.07\textwidth}|P{0.07\textwidth}|P{0.07\textwidth}|P{0.07\textwidth}|P{0.07\textwidth}}
\multicolumn{10}{c}{\textbf{Desktop}} \\
\bottomrule
% \multicolumn{10}{c}{Global Distributions} \\
% \bottomrule
\textbf{Experiment} & \makecell{\textbf{Global}\\ \textbf{STD$\downarrow$ (\%)}} & \makecell{\textbf{Global}\\ \textbf{SER}$\downarrow$} & \makecell{\textbf{Mean P.-S.}\\ \textbf{STD$\downarrow$ (\%)}} & \makecell{\textbf{Mean P.-S.}\\ \textbf{SER$\downarrow$}} & \textbf{FDR$\uparrow$} & \textbf{IR$\downarrow$} & \textbf{GARBE$\downarrow$}  & \textbf{SIR$_{a}$ (\%) $\downarrow$} & \textbf{SIR$_{g}$ (\%) $\downarrow$} \\
\bottomrule
TypeNet, \textit{5F}  & \textbf{0.27} & 1.34 & \textbf{0.49} & 3.27 & 0.95 & 1.39 & 0.07  & 2.92 & 2.23 \\
TypeNet, \textit{4F} & 0.4 & 1.38 & 0.61 & 2.89 & 0.93 & 1.43 & 0.07 & \textbf{2.62} & 2.12  \\
TypeNet, \textit{10F} & 0.4 & 1.37 & 0.6 & 2.85 & 0.95 & 1.43 & 0.07  & \textbf{2.62} & \textbf{2.02}\\
TypeNet, \textit{11F} & 0.28 & 1.36 & 0.55 & 3.38  & 0.94 & 1.53 & 0.07 & 3.05 & 2.25 \\
\hline
TypeFormer, \textit{5F} & 0.53 & 1.26 & 0.76 & \textbf{2.04} & \textbf{0.98} & 1.3 & 0.05 & 3.14 & 2.65 \\
TypeFormer, \textit{4F}  & 0.6 & 1.27 & 0.78 & 2.05& \textbf{0.98} & \textbf{1.18} & \textbf{0.03}  & 2.97 & 2.45 \\
TypeFormer, \textit{10F} & 0.47 & \textbf{1.23} & 0.79 & 2.1 & 0.97 & 1.2 & 0.04  & 2.97 & 2.49 \\
TypeFormer, \textit{11F} & 0.61 & 1.31 & 0.75 & \textbf{2.04} & \textbf{0.98} & 1.4 & 0.07 & 3.16 & 2.52 \\

\bottomrule
% \multicolumn{7}{c}{Per-Subject Average Distributions} \\
% \bottomrule
% & STD & SER & SIR & GARBE & FDR & IR & & & \\
% \bottomrule
% TypeNet, \textit{5F} & & & & & & & & \\
% TypeNet, \textit{4F} & & & & & & & & & \\
% TypeNet, \textit{10F} & & & & & & & & & \\
% TypeNet, \textit{11F} & & & & & & & & & \\
% \hline
% TypeFormer, \textit{5F} & & & & & & & & & \\
% TypeFormer, \textit{4F} & & & & & & & & & \\
% TypeFormer, \textit{10F} & & & & & & & & & \\
% TypeFormer, \textit{11F} & & & & & & & & & \\
% \bottomrule

\end{tabular}

\begin{tabular}
{P{0.11\textwidth}|P{0.07\textwidth}|P{0.07\textwidth}|P{0.07\textwidth}|P{0.07\textwidth}|P{0.07\textwidth}|P{0.07\textwidth}|P{0.07\textwidth}|P{0.07\textwidth}|P{0.07\textwidth}}
\multicolumn{10}{c}{\textbf{Mobile}} \\
\bottomrule
% \multicolumn{10}{c}{Global Distributions} \\
% \bottomrule
% & \makecell{\textbf{Global}\\ \textbf{STD (\%)}} & \makecell{\textbf{Global}\\ \textbf{SER}} & \makecell{\textbf{Mean Per-}\\ \textbf{Subject STD (\%)}} & \makecell{\textbf{Mean Per-}\\ \textbf{Subject SER}} & \makecell{\textbf{SIR_{age}}\\ \textbf{(\%)}} & \makecell{\textbf{SIR_{gender}}\\ \textbf{(\%)}} & GARBE & FDR & IR \\
\textbf{Experiment} & \makecell{\textbf{Global}\\ \textbf{STD$\downarrow$ (\%)}} & \makecell{\textbf{Global}\\ \textbf{SER}$\downarrow$} & \makecell{\textbf{Mean P.-S.}\\ \textbf{STD$\downarrow$ (\%)}} & \makecell{\textbf{Mean P.-S.}\\ \textbf{SER$\downarrow$}} & \textbf{FDR$\uparrow$} & \textbf{IR$\downarrow$} & \textbf{GARBE$\downarrow$}  & \textbf{SIR$_{a}$ (\%) $\downarrow$} & \textbf{SIR$_{g}$ (\%) $\downarrow$} \\
\bottomrule
TypeNet, \textit{5F}& 1.36 & 1.93 & 1.61 & 3.15& \textbf{0.96} & \textbf{2.09}  & \textbf{0.1} & 6.71 & 8.3   \\
TypeNet, \textit{4F} & 1.22 & 1.5 & 1.54 & 2.48 & 0.95 & 3.41 & 0.18 & \textbf{2.88} & \textbf{3.52}  \\
TypeNet, \textit{10F} & 1.12 & 1.62 & 1.56 & 2.6 & 0.95 & 2.45 & 0.17  & 4.21 & 5.15  \\
TypeNet, \textit{11F} & \textbf{0.62} & \textbf{1.29} & 1.15 & \textbf{2.26} & 0.95 & 2.36 & \textbf{0.1}  & 7.08 & 8.72 \\
\hline
TypeFormer, \textit{5F}& 0.95 & 1.73 & \textbf{1.03} & 2.76 & 0.95 & 2.11 & 0.14 & 6.9 & 7.57  \\
TypeFormer, \textit{4F} & 1.14 & 1.56 & 1.31 & 2.43 & \textbf{0.96} & 2.52 & 0.14 & 6.43 & 6.26 \\
TypeFormer, \textit{10F} & 0.78 & 1.48 & 1.26 & 2.62 & 0.95 & 2.34 & 0.16  & 6.44 & 6.1\\
TypeFormer, \textit{11F} & 1.19 & 1.84 & 1.38 & 2.73 & 0.94 & 2.25 & 0.12 & 7.6 & 7.4 \\

\bottomrule
% \multicolumn{7}{c}{Per-Subject Average Distributions} \\
% \bottomrule
% & STD & SER & SIR & GARBE & FDR & IR \\
% \bottomrule
% TypeNet, \textit{5F} & & & & & \\
% TypeNet, \textit{4F} & & & & & & \\
% TypeNet, \textit{10F} & & & & & & \\
% TypeNet, \textit{11F} & & & & & & \\
% \hline
% TypeFormer, \textit{5F} & & & & & & \\
% TypeFormer, \textit{4F} & & & & & & \\
% TypeFormer, \textit{10F} & & & & & & \\
% TypeFormer, \textit{11F} & & & & & & \\
% \bottomrule

\end{tabular}

\vspace{0.2cm}
\label{tab:demographic_metrics}
\end{table*}


\subsection{Fairness Evaluation}
Table \ref{tab:glob_eer_dem} shows the performance in terms of global EER (\%) considering different demographic groups. Age groups are placed along the rows, while genders along the columns. As an example, from all experiments we take into consideration TypeNet in the desktop case, and TypeFormer in the mobile case, based on the same set of features (``5F''). In both cases, it is possible to see that males achieved lower error rates (6.50\% against 7.11\% of global EER for TypeNet, and 9.62\% against 10.37\% for TypeFormer, respectively for males and females). It is interesting to notice that, although the STD and SER values are quite smaller in the desktop case, the difference of EER between error rates across genders is still significant. Formulating an hypothesis that would explain this trend is not immediate, and out of the scope of the current work. Furthermore, by analyzing the behavior of the systems considering different age groups, it is possible to notice that for younger subjects, TypeFormer performs worse than for older ones, while this trend is not as evident for TypeNet. Such discrepancy could be due to cultural differences related to the degree of easiness and comfort in interacting with mobile devices across different generations. 
%Moreover, while in the type of 

Table \ref{tab:demographic_metrics} shows all results of the fairness assessment provided throughout the proposed framework. Along the rows, the table is divided into two parts: the upper part presents the results in the desktop scenario, while the lower part is focused on the mobile scenario. Each half is further divided into two sections, each reporting results of one of the two models considered, TypeNet and TypeFormer, considering the four experimental configurations presented in Sec. \ref{subsec:evaluation}. Concerning the different metrics, it is necessary to point out that all metrics except $\textrm{SIR}$ are calculated considering 12 demographic groups, due to 6 age groups and 2 genders (see Sec. \ref{sec:resources}). In contrast, $\textrm{SIR}_{a}$ is computed considering scores divided by age only (square matrix of dimension 6), while $\textrm{SIR}_{g}$ considering gender only (square matrix of dimension 2), to keep the assessments of each of the two attributes independent (Sec. \ref{sec:metrics}).

By observing Table \ref{tab:demographic_metrics}, it possible to notice that there is no clear superiority of one model as in the case of the verification performance (TypeNet \textit{5F} for desktop devices, TypeFormer \textit{10F} for mobile devices). 
By carrying out an overall comparison of the desktop and mobile scenarios, it is possible to observe that demographic differentials related to age and gender tend to be higher in the mobile case. In fact, considering the mean values for each one of the metrics computed over all desktop against all mobile experiments, we obtain global STD 0.45\% vs 1.05\%, global SER 1.32 vs 1.62, mean per-subject STD 0.67\% vs 1.36\%, mean per-subject SER 2.58 vs 2.63, FDR 0.96 vs 0.95, IR 1.36 vs 2.44, GARBE 0.06 vs 0.14, SIR$_{a}$ 2.93\% vs 6.03\%, SIR$_{g}$ 2.34\% vs 6.63\%. It is clear that in the desktop scenario there is an improvement in fairness according to each single metric. 



If we consider a comparison of the two architectures in each scenario, we can see that in the desktop case the average performance achieved by TypeNet in terms of SIR$_{a}$ is 2.80\% and SIR$_{g}$ is 2.16\%, while the scores of TypeFormer are respectively 3.06\% and 2.53\%, being more biased as well as less effective. A similar trend is reported for the mobile case, with TypeNet (although with lower verification performance) achieving SIR$_{a}$=5.22\% and SIR$_{g}$=6.42\%, against SIR$_{a}$=6.84\% and SIR$_{g}$=6.83\% achieved by TypeFormer.

Finally, having a look at trends due to different sets of input features within the same scenario and same model configuration, we can observe that the results are more irregular and they do not show a clear overall trend as in the previous cases. Nevertheless, considering for instance the SIR values, we can observe that generally the ASCII code is associated with higher bias in almost all experiments and scenarios, showing that comparisons among the same demographic groups are slightly harder than among different groups. %In the desktop case, for TypeNet, a slight but opposite trend is visible for metrics such as global and mean per-subject STD, suggesting that, although comparisons among the same demographic groups are slightly harder than among different groups, the system does not perform equally well within the same group for all groups.





% \begin{table}[b]
% \centering
% \caption{Complete comparison of the presented keystroke biometric recognition systems.}
% \begin{tabular}{c|c|c|c}
% \bottomrule
% \multicolumn{4}{c}{\textbf{Desktop}} \\
% \bottomrule
% Metric & \makecell[c]{\textbf{Baseline}\\ \textbf{RNN}}  & \makecell[c]{\textbf{TypeNet}\\ \textbf{\cite{typenet}}} & \makecell[c]{\textbf{TypeFormer}\\ \textbf{\cite{typeformer}}} \\   
% \hline
% \multicolumn{4}{c}{Global Distributions} \\
% \hline
% \textbf{EER (\%)} & 25.03\% & 6.76\% & 12.41\% \Tstrut\\
% \makecell{\textbf{Accuracy}\\  \textbf{(\%)}} & 74.97\% & 93.24\% & 87.59\%  \Tstrut\\
% \makecell{\textbf{AUC}\\  \textbf{(\%)}} & 82.60\% & 98.08\% & 94.50\% \Tstrut\\
% \textbf{TAR @1\% FAR} \Tstrut\Bstrut & 4.18\% & 60.43\%& 26.45\% \\
% \hline
% \multicolumn{4}{c}{Per-Subject Distributions (Mean Values)} \\
% \hline
% \textbf{EER (\%)} \Tstrut & 21.20\% & 2.71\% & 7.27\% \\
% \makecell{\textbf{Accuracy}\\  \textbf{(\%)}} \Tstrut & 74.97\% & 95.31\% & 91.54\%\\
% \makecell{\textbf{AUC}\\  \textbf{(\%)}} \Tstrut & 82.60\% & 99.26\% & 96.77\%\\
% % \textbf{TAR @1\% FAR} \Tstrut & - & - & -\\
% \bottomrule
% \end{tabular}


% \begin{tabular}{c|c|c|c}
% \multicolumn{4}{c}{\textbf{Mobile}} \\
% \bottomrule
% Metric & \makecell[c]{\textbf{Baseline}\\ \textbf{RNN}}  & \makecell[c]{\textbf{TypeNet}\\ \textbf{\cite{typenet}}} & \makecell[c]{\textbf{TypeFormer}\\ \textbf{\cite{typeformer}}} \\      
% \hline
% \multicolumn{4}{c}{Global Distributions} \\
% \hline
% \textbf{EER (\%)} & 33.34\% & 13.95\% & 9.34\%\Tstrut\\
% \makecell{\textbf{Accuracy}\\  \textbf{(\%)}} & 66.66\% & 86.05\% & 90.66\% \Tstrut\\
% \makecell{\textbf{AUC}\\  \textbf{(\%)}} & 73.77\% & 93.81\% & 96.33\% \Tstrut\\
% \textbf{TAR @1\% FAR} \Tstrut\Bstrut & 2.73\% & 29.95\% & 32.04\% \\
% \hline
% \multicolumn{4}{c}{Per-Subject Distributions (Mean Values)} \\
% \hline
% \textbf{EER (\%)} \Tstrut &  32.93\% & 8.00\% & 5.35\%\\
% \makecell{\textbf{Accuracy}\\  \textbf{(\%)}} \Tstrut & 67.58\% & 90.89\% & 93.11\%\\
% \makecell{\textbf{AUC}\\  \textbf{(\%)}} \Tstrut & 74.60\% & 96.43\% & 97.77\%\\
% % \textbf{TAR @1\% FAR} \Tstrut & - & - & -\\
% \bottomrule
% \end{tabular}
% \vspace{0.2cm}
% \label{tab:all_metrics}
% \end{table}





% \begin{table}[hb!]
% \caption{Identification performance for each of the cases presented.}
% \centering
% \begin{tabular}{|c|c|c||c|c|c|}
% \multicolumn{6}{c}{\textbf{Baseline RNN}} \\
% \multicolumn{3}{c}{\textbf{Desktop}} & \multicolumn{3}{c}{\textbf{Mobile}} \\
% \hline
%  \textbf{Rank-1} & \textbf{Rank-3} & \textbf{Rank-5} &  \textbf{Rank-1} & \textbf{Rank-3} & \textbf{Rank-5} \\
% \hline
%  23.17\% & 55.95\% & 75.81\% & 10.71\% & 30.07\% & 49.30\% \\
% \hline
% \end{tabular}
% \vspace{.3cm}


% \begin{tabular}{|c|c|c||c|c|c|}
% \multicolumn{6}{c}{\textbf{TypeNet \cite{typenet}}} \\
% \multicolumn{3}{c}{\textbf{Desktop}} & \multicolumn{3}{c}{\textbf{Mobile}} \\
% \hline
%  \textbf{Rank-1} & \textbf{Rank-3} & \textbf{Rank-5} &  \textbf{Rank-1} & \textbf{Rank-3} & \textbf{Rank-5} \\
% \hline
%  89.81\% & 99.03\% & 99.79\% & 68.50\% & 90.60\% & 96.41\% \\
% \hline
% \end{tabular}
% \vspace{.3cm}

% \begin{tabular}{|c|c|c||c|c|c|}
% \multicolumn{6}{c}{\textbf{TypeFormer \cite{typeformer}}} \\
% \multicolumn{3}{c}{\textbf{Desktop}} & \multicolumn{3}{c}{\textbf{Mobile}} \\
% \hline
%  \textbf{Rank-1} & \textbf{Rank-3} & \textbf{Rank-5} &  \textbf{Rank-1} & \textbf{Rank-3} & \textbf{Rank-5} \\
% \hline
%   67.08\% & 92.49\% & 97.78\% & 74.02\% & 95.70\% & 98.95\% \\
% \hline
% \end{tabular}
% \vspace{.3cm}
% \label{tab:identification}
% \end{table}



% \subsection{Demographic Differentials}

% Additionally, we will exploit the scores to assess possible demographic differentials (based on gender and age). To this end, the comparisons between sessions of the evaluation set are designed to highlight such possible effects. The results of this assessment will be included in the competition summary paper as well. Table \ref{table:bias} reports the global EER by subject demographic group for Task 1 (Desktop) and for Task 2 (Mobile). It is possible to notice that the error rates are higher for younger subjects and for females. Table \ref{table:sims} displays the average impostor scores considering enrolment sessions along the rows and verification subject sessions along the columns, grouped by age (left) and gender (right). In the vast majority of the cases, the scores results higher along the main diagonal (or closer to it), showing that \textbf{impostors belonging to the same demographic group are harder to distinguish}. Consequently, \textbf{some demographic information is retained in the scores} for the evaluated system. The matrix is symmetrical. For brevity, we include only the results for Task 2 (Mobile). \textbf{Additional metrics} quantifying the demographic information in the scores \textbf{might be included at a later time}, such as the Fairness Discrepancy Rate (FDR) \cite{9507539} to enrich the system assessment provided by participating in the competition.



% \begin{table}[hb!]
% \caption{Increase of average impostor similarity considering same vs different demographic group.}
% \centering
% \begin{tabular}{c|c|c}
% System & Age & Gender \\
% \hline
% \multicolumn{3}{c}{\textbf{Desktop}} \\
% \hline
% \textbf{Baseline RNN} & 0.93\% & 0.67\% \\
% \textbf{TypeNet \cite{typenet}} & 2.92\% & 2.23\%\\
% \textbf{TypeFormer \cite{typeformer}} & 3.22\% & 2.74\% \\
% \hline
% \multicolumn{3}{c}{\textbf{Mobile}} \\
% \hline
% \textbf{Baseline RNN} & 3.84\% & 5.06\% \\
% \textbf{TypeNet \cite{typenet}}  & 6.71\% & 8.30\%\\
% \textbf{TypeFormer \cite{typeformer}} & 7.18\% & 7.66\%\\
% \hline
% \end{tabular}
% \vspace{.3cm}
% \end{table}

% \begin{table}
% \textbf{Skewed Impostor Similarity Ratio (SIR)}
% \vspace{0.2cm}

% % \begin{minipage}{.5\linewidth}
% \centering
% \begin{tabular}{c|c}
% \textbf{System} & \textbf{SIR} \\
% \hline
% TypeNet Desktop Age & 2.92\%\\
% TypeNet Desktop Gender & 2.23\%\\
% TypeFormer Mobile Age & 7.18\%\\
% TypeFormer Mobile Gender & 7.66\%\\
% \hline
% \end{tabular}
% % \end{minipage}
% \vspace{0.2cm}
%  \caption{\small Impostor scores obtained considering enrolment sessions along the rows and verification subject sessions along the columns, grouped by age (left) and gender (right) for Task 2 (Mobile).}
%  \label{table:sims}
% \end{table}


% \begin{table}
% \textbf{Average Impostor Distances by Demographic Group}
% \textbf{TypeNet \cite{typenet} - Desktop} \\
% \vspace{0.2cm}

% % \begin{minipage}{.5\linewidth}
% \centering
% \textbf{Age}
% \begin{tabular}{c|cccccc}
% \bottomrule
%  & \textbf{10-13}  &  \textbf{14-17}
% & \textbf{18-26}  &  \textbf{27-35}
% & \textbf{36-44}  &  \textbf{44-79}\\   
% \hline
% \textbf{10 - 13} & 0.319 & 0.307 & 0.306 & 0.303 & 0.301 & 0.3 \Tstrut\\
% \textbf{14 - 17} & 0.307 & 0.317 & 0.312 & 0.312 & 0.310 & 0.306 \Tstrut\\
% \textbf{18 - 26} & 0.306 & 0.312 & 0.311 & 0.311 & 0.308 & 0.308 \Tstrut\\
% \textbf{27 - 35} & 0.303 & 0.312 & 0.311 & 0.317 & 0.310 & 0.311 \Tstrut\\
% \textbf{36 - 44} & 0.301 & 0.310 & 0.308 & 0.310 & 0.317 & 0.316 \Tstrut\\
% \textbf{45 - 79} & 0.3 & 0.306 & 0.308 & 0.311 & 0.316 & 0.321 \Tstrut\Bstrut\\
% \bottomrule
% \multicolumn{7}{c}{\textbf{P}: 2.92\%}\\
% \bottomrule

% \end{tabular}
% % \end{minipage}
% % \hfill
% % \begin{minipage}{.3\linewidth}
% \centering
% \textbf{Gender}\\
% \vspace{.05cm}
% \begin{tabular}{c|cc}
% \bottomrule
% & \textbf{Male}  &  \textbf{Female}\\   
% \hline
% \textbf{Male} & 0.315 & 0.309 \Tstrut\\
% \textbf{Female} & 0.309 & 0.317 \Tstrut\Bstrut\\
% \bottomrule
% \multicolumn{3}{c}{\textbf{P}: 2.23\%}\\
% \bottomrule
% \end{tabular}
% % \end{minipage}
% \vspace{0.2cm}



% \textbf{TypeFormer \cite{typeformer}} \\
% \vspace{0.2cm}
% % \begin{minipage}{.5\linewidth}
% \centering
% \textbf{Age}
% \begin{tabular}{c|cccccc}
% \bottomrule
%  & \textbf{10-13}  &  \textbf{14-17}
% & \textbf{18-26}  &  \textbf{27-35}
% & \textbf{36-44}  &  \textbf{44-79}\\   
% \hline
% \textbf{10 - 13} & 0.436 & 0.430 & 0.404 & 0.404 & 0.385 & 0.388 \Tstrut\\
% \textbf{14 - 17} & 0.430 & 0.447 & 0.401 & 0.400 & 0.384 & 0.367 \Tstrut\\
% \textbf{18 - 26} & 0.404 & 0.401 & 0.431 & 0.399 & 0.394 & 0.381 \Tstrut\\
% \textbf{27 - 35} & 0.404 & 0.400 & 0.399 & 0.420 & 0.401 & 0.388 \Tstrut\\
% \textbf{36 - 44} & 0.385 & 0.384 & 0.394 & 0.401 & 0.412 & 0.409 \Tstrut\\
% \textbf{45 - 79} & 0.388 & 0.367 & 0.381 & 0.388 & 0.409 & 0.398 \Tstrut\Bstrut\\
% \bottomrule
% \multicolumn{7}{c}{\textbf{P}: 7.18\%}\\
% \bottomrule
% \end{tabular}
% % \end{minipage}
% % \hfill
% % \begin{minipage}{.3\linewidth}
% \centering
% \textbf{Gender}\\
% \vspace{.05cm}
% \begin{tabular}{c|cc}
% \bottomrule
% & \textbf{Male}  &  \textbf{Female}\\   
% \hline
% \textbf{Male} & 0.425 & 0.389 \Tstrut\\
% \textbf{Female} & 0.389 & 0.410 \Tstrut\Bstrut\\
% \bottomrule
% \multicolumn{3}{c}{\textbf{P}: 7.66\%}\\
% \bottomrule
% \end{tabular}
% % \end{minipage}
% \vspace{0.2cm}
%  \caption{\small Impostor scores obtained considering enrolment sessions along the rows and verification subject sessions along the columns, grouped by age (left) and gender (right) for Task 2 (Mobile).}
%  \label{table:sims}
% \end{table}
